Emergence, Formation and Dynamics of Hot QCD Matter

In this thesis, we make progress in two concrete directions in the vast landscape of hot QCD physics. The first one is quarkonium transport inside quark-gluon plasma (QGP), the high temperature phase of QCD. Over the past two decades it has been realized that a significant fraction of quarkonium suppression in high energy heavy ion collisions comes from dynamic dissociation and recombination processes, instead of static screening of the interaction potential as originally proposed by Matsui and Satz. Our contribution is the formulation of the precise correlation functions in QCD at finite temperature that describe the dissociation and recombination processes of heavy quarkonium in QGP, as well as their calculation in weakly coupled QCD and strongly coupled $\mathcal{N}=4$ supersymmetric Yang-Mills theory. We also formulate the Euclidean version of these correlation functions so that they may be calculated using Lattice QCD techniques. The second contribution we make is the development of tools to understand the process of hydrodynamization in QCD kinetic theory and their application to a simplified description where only a subset of the QCD scattering mechanisms are included. By doing this, we learn that the process of hydrodynamization in this theory, and specifically, how memory of the initial condition is lost, follows the recently proposed Adiabatic Hydrodynamization scenario. Concretely, hydrodynamization proceeds through a sequential process in which a monotonously shrinking set of low-energy states dominate the dynamics, where the opening of an energy gap relative to the ground state(s) signals the start of each stage of this process. The hydrodynamic attractor is reached when only one low-energy state remains as the ground state, and the system approaches local thermal equilibrium following the adiabatic evolution of this low-energy state.

==> biography.tex <==
%% This section is optional

\chapter*{Biographical Sketch}
\addcontentsline{toc}{chapter}{\protect\textbf{Biographical Sketch}}

%Silas Whitcomb Holman was born in Harvard, Massachusetts on January 20, 1856. He received his S.B. degree in Physics from MIT in 1876, and then joined the MIT Department of Physics as an Assistant. He became Instructor in Physics in 1880, Assistant Professor in 1882, Associate Professor in 1885, and Full Professor in 1893. Throughout this period, he struggled with increasingly severe rheumatoid arthritis. At length, he was defeated, becoming Professor Emeritus in 1897 and dying on April 1, 1900.

%Holman's light burned brilliantly before his tragic and untimely death. He published extensively in thermal physics, and authored textbooks on precision measurement, fundamental mechanics, and other subjects. He established the original Heat Measurements Laboratory. Holman was a much admired teacher among both his students and his colleagues. The reports of his department and of the Institute itself refer to him frequently in the 1880's and 1890's, in tones that gradually shift from the greatest respect to the deepest sympathy.

%Holman was a student of Professor Edward C. Pickering, then head of the Physics department. Holman himself became second in command of Physics, under Professor Charles R. Cross, some years later. Among Holman's students, several went on to distinguish themselves, including: the astronomer George E. Hale ('90) who organized the Yerkes and Mt. Wilson observatories and who designed the 200 inch telescope on Mt. Palomar; Charles G. Abbot ('94), also an astrophysicist and later Secretary of the Smithsonian Institution; and George K. Burgess ('96), later Director of the Bureau of Standards. 

==> fontsets/mitthesis-defaultfonts.tex <==
% From mitthesis package
% Version: 1.02, 2023/07/03
% Documentation: https://ctan.org/pkg/mitthesis

%% Default fonts
%
\ifpdftex
	\typeout{^^JLoading Computer Modern text and math fonts (default for pdftex).^^J}
	\RequirePackage[T1]{fontenc}
	\RequirePackage{bm}
\else
	\typeout{^^JLoading Latin Modern text and math fonts (default for unicode engines).^^J}
	%
    \RequirePackage[warnings-off={mathtools-colon,mathtools-overbracket}]{unicode-math}
    % suppress tiresome warnings about lack of integration between mathtools and unicode-math.
    % Unicode-math loads fontspec package, but default fonts are not selected by fontspec in this case.
\fi


==> fontsets/mitthesis-fira-newtxsf.tex <==
% From mitthesis package
% Version: 1.02, 2023/07/03
% Documentation: https://ctan.org/pkg/mitthesis


%% Fira Sans text font with newtx sans serif math font and Inconsolata typewriter font
%
\ifpdftex
	\typeout{^^JLoading Fira sans text font with newtx sans serif math font and Inconsolata typewriter^^J}
    \RequirePackage[sfdefault]{FiraSans} % sans serif text package %,scaled=.85
	\RequirePackage[T1]{fontenc}
    \RequirePackage[varqu,varl,,scaled=1.12]{zi4} % inconsolata font for typewriter
    \RequirePackage[cmintegrals,scaled=1.12]{newtxsf} % sans serif math
 	\RequirePackage{bm}
\else
	\ClassWarning{mitnewthesis}{The newtx font set requires pdflatex. Defaulting to LMR fonts}
    \RequirePackage[warnings-off={mathtools-colon,mathtools-overbracket}]{unicode-math}
    % suppress tiresome warnings about lack of integration between mathtools and unicode-math.
    % Unicode-math loads the fontspec package, but the default fonts are not selected by fontspec in this case.
\fi


==> fontsets/mitthesis-heros-stix2.tex <==
% From mitthesis package
% Version: 1.01, 2023/07/03
% Documentation: https://ctan.org/pkg/mitthesis


%% TeX Gyre Heros (sans serif) text font with STIX Two Math font and Inconsolata monospaced font
%
% These fonts are available at: 
%				http://www.gust.org.pl/projects/e-foundry/tex-gyre 
%				https://github.com/stipub/stixfonts 
%				https://ctan.org/tex-archive/fonts/inconsolata
% Install these as system fonts on your computer
%
\ifpdftex
	\ClassWarning{mitnewthesis}{The heros-stix2 fontset requires a unicode engine. Defaulting to CMR fonts.}
	\RequirePackage[T1]{fontenc}
	\RequirePackage{bm}
\else
	\typeout{^^JTeX Gyre Heros (sans serif) text font with STIX2 math font and Inconsolata monospaced font.^^J}
	%
    \RequirePackage[warnings-off={mathtools-colon,mathtools-overbracket}]{unicode-math}
    % suppress tiresome warnings about lack of integration between mathtools and unicode-math
    % unicode-math loads the fontspec package

    \setmainfont{texgyreheros}[% Presumes these are system fonts! Available at: http://www.gust.org.pl/projects/e-foundry/tex-gyre
		WordSpace = {1,1.4,1},
		Extension = .otf,
    	UprightFont = *-regular,
    	ItalicFont = *-italic,
    	BoldFont = *-bold,
    	BoldItalicFont = *-bolditalic,
		Numbers = Lining,
    	Scale=0.91,
	]        
    \setsansfont{texgyreheros}[% Presumes these are system fonts! Available at: http://www.gust.org.pl/projects/e-foundry/tex-gyre
		WordSpace = {1,1.4,1},
		Extension = .otf,
    	UprightFont = *-regular,
    	ItalicFont = *-italic,
    	BoldFont = *-bold,
    	BoldItalicFont = *-bolditalic,
		Numbers = Lining,
    	Scale=0.91,
	]        
   \setmonofont{Inconsolatazi4}[% This otf font ships with the LaTeX Inconsolata package and is in CTAN https://ctan.org/tex-archive/fonts/inconsolata
        Scale=1.05,
        Extension = .otf,
        UprightFont = *-Regular,
        ItalicFont = *-Regular,% has no italic face
        BoldFont = *-Bold, 
    	BoldItalicFont = *-Bold,% has no bold italic face
        RawFeature = {+ss01,+ss02,+ss03},
    ]             
    \setmathfont{STIXTwoMath-Regular}[% nice glyphs, but \mkern sometimes needed %% https://github.com/stipub/stixfonts
    	Scale=MatchUppercase,
    	Extension = .otf,
		BoldFont = *,% STIX Two Math has no bold face
%       Color=NavyBlue, 
    	RawFeature = {+ss01, -ss02, -ss08},
    ]
    % ss01 -- switch calligraphic to script; +ss02 -- variants of g, u, v, w, z; +ss08 -- upright integrals
    %    
    \setmathfontface\mathbf{STIXTwoText-Bold.otf}[]% to not get Heros bold, https://github.com/stipub/stixfonts
    \setmathfontface\mathit{STIXTwoText-Italic.otf}[]
    \setmathfontface\mathrm{STIXTwoText-Regular.otf}[]% to get roman letters from STIX Two
     %         
    \newcommand*{\FRAC}[1]{{\addfontfeature{Fractions=On}#1}}% use OpenType feature for fractions, \FRAC{1/2} 
\fi


==> fontsets/mitthesis-libertine.tex <==
% From mitthesis package
% Version: 1.01, 2023/07/03
% Documentation: https://ctan.org/pkg/mitthesis

%% Linux Libertine (serif) text font with newtxmath[libertine] (pdftex) or Libertinus (unicode) math font
%
%  These fonts are available here https://ctan.org/tex-archive/fonts/libertine/opentype 
%						 and here https://github.com/alerque/libertinus
% install these as system fonts on your computer
%
\ifpdftex
	\typeout{^^JLoading newtx-libertine text and math fonts with insolata typewriter font^^J}
    \RequirePackage[lining,semibold]{libertine} 
    \RequirePackage[T1]{fontenc}
    \RequirePackage[varqu,varl]{inconsolata}% typewriter
%    \usepackage{amsthm}% must be loaded before newtxmath
    \RequirePackage[libertine,vvarbb]{newtxmath}
    \RequirePackage{bm}% load after all math to give access to bold math
\else
	\typeout{^^JLoading Linux Libertine (serif) text font with Libertinus math font^^J}
	%
    \RequirePackage[warnings-off={mathtools-colon,mathtools-overbracket}]{unicode-math}
    % suppress tiresome warnings about lack of integration between mathtools and unicode-math
    % unicode math loads the fontspec package
 	%
    \setmainfont{LinLibertine}[% Linux Libertine O  
    	Extension = .otf,
    	UprightFont = *_R,
    	ItalicFont = *_RI,
    	BoldFont = *_RZ, % Libertine O Semibold
    	BoldItalicFont = *_RZI, % Libertine O Semibold Italic
    %	Ligatures=Rare,% TeX
    %	Numbers=OldStyle,%
    	RawFeature={+ss05},% +ss02 would change J, K, R; +ss05 changes W	
        ]    
    \setmonofont{LinLibertine}[% Linux Libertine Mono O
    	Scale=0.9,
	    Extension = .otf,
    	UprightFont = *_M,
    	ItalicFont = *_MO,% oblique
    	BoldFont = *_MB,
	    BoldItalicFont = *_MBO,% oblique
	]    
    \setsansfont{LinBiolinum}[% Linux Biolinum O
    	Extension = .otf,
    	UprightFont = *_R,
    	ItalicFont = *_RI,
    	BoldFont = *_RB,
	    BoldItalicFont = *_RBO,% oblique
    	Scale=MatchUppercase]
	%    	
    %% a Libertine-style math font
    \setmathfont{libertinusmath-regular}[%
     	Extension = .otf,   
    	Scale=MatchUppercase,
		BoldFont = *,% This font lacks a bold version
    	RawFeature={+ss08},% +ss08 gives slanted integrals (no other features) 	
    	]
    \newcommand*{\FRAC}[1]{{\addfontfeature{Fractions=On}#1}}% use OpenType feature for fractions, \FRAC{1/2}   
\fi


==> fontsets/mitthesis-lucida.tex <==
% From mitthesis package
% Version: 1.01, 2023/07/03
% Documentation: https://ctan.org/pkg/mitthesis


%% Lucida Bright and Lucida Bright Math fonts (available from the TeX Users Group)

\typeout{^^JLucida Bright and Lucida Bright Math fonts^^J}

\ifpdftex
	\RequirePackage[LY1]{fontenc}
	\RequirePackage[expert,vargreek,altbullet,seriftt]{lucidabr}   % switch text and math fonts
	\RequirePackage{bm}
\else
    \RequirePackage[warnings-off={mathtools-colon,mathtools-overbracket}]{unicode-math}
    % suppress tiresome warnings about lack of integration between mathtools and unicode-math
    % unicode-math loads the fontspec package

    % FEATURE 	DESCRIPTION 											DEFAULT
    % dlig 		discretionary ligatures (f-ligatures in typewriter fnt) off
    % liga 		standard ligatures (f-ligatures, not monospaced fonts) 	on
    % onum 		old style numbers (Lucida Bright only)					off
    % smcp 		small caps 	(Lucida Bright, upright only)				off
    % zero 		slashed zero (sans and monospaced fonts)				off
    % locl 		script/language specific (localized) forms 				on
    %
    % FEATURE 	FONT 						DESCRIPTION
    % ss01 		Lucida Sans & Typewriter 	use dotted zero: 𝟶 vs. default 0.
    % ss01 		use Lucida-standard shapes:
    % 			Lucida Grande Mono 			ØOQ vs. default 0OQ;
    % 			Lucida Console 				ØOQ vs. default 0OQ.
    
    \setmainfont{LucidaBrightOT}[% main rm
          Ligatures=TeX,
          Extension=.otf,
          UprightFont=*,
          ItalicFont=*-Italic,
          BoldFont=*-Demi,
    	  BoldItalicFont=*-DemiItalic,
          BoldItalicFeatures={Color=Purple4},
    %     UprightFeatures={Color=Salmon3},
    	  Scale=0.92,
    %	  Numbers ={OldStyle}, 
      ]
    %
    \setsansfont{LucidaSansOT}[% main sans
          Ligatures=TeX,
          Extension=.otf,
          UprightFont=*,
          ItalicFont=*-Italic,
          BoldFont=*-Demi,
    	  BoldItalicFont=*-DemiItalic,
    	  Scale=MatchUppercase,
      ]
    %
    \setmonofont{LucidaSansTypewriterOT}[% main typewriter
          Ligatures=TeX,
          Extension=.otf,
          UprightFont=*,
          ItalicFont=*-Oblique,
          BoldFont=*-Bold,
          BoldItalicFont=*-BoldOblique,
      	  Scale=MatchUppercase,
      ]
    
    %% MATH FONTS
    %
    % ss01 	alternate Latin lower case math italic identical to text italic. This option is not recommended as Greek 𝜈 (nu) and Latin 𝑣 (vee) become too similar
    % ss02 	smaller arrows (original Type 1 size): ⇑ vs. default ⇑.
    % ss03 	attempt to imitate Type 1 fonts
    % ss04 	calligraphic alternative (similar to the Type 1 design) to the math script alphabet
    % ss05 	use a slashed-zero style for the empty set character (U+2205): Ø vs. default ∅
    % ss08 	emphasize right and bottom edges of the d’Alembertian operator (U+29E0, \laplac), to follow the design of the Laplace operator (U+2206, \increment, Δ); the default design emphasizes the left and upper edges. Also available in the bold math font.
    %
    \setmathfont{LucidaBrightMathOT}[% main math
    	  Scale=MatchUppercase,
    	  Extension=.otf,
    	  BoldFont=LucidaBrightMathOT-Demi.otf,
%    	  BoldFeatures={Color=Chartreuse4},
    	  RawFeature ={+ss04,+ss08}, %
    ]
 
%% LucidaMath-OT contains a *serif* typerwriter font. If you prefer a sans serif typerwriter font, you can use the following two settings. 
% 
%    \setmathfont{LucidaSansTypewriterOT}[% <== NB: setting a text font where math font should go.
%    	  Scale=MatchUppercase,
%          range=tt,
%    	  Color=NavyBlue,
%          Extension=.otf,
%          script-features = {},     
%          sscript-features = {},     
%    	  BoldFont=LucidaSansTypewriterOT-Bold.otf,
%    	  BoldFeatures={Color=Salmon3},
%    ]
%    %
%    \setmathfontface\mathtt{LucidaSansTypewriterOT-Bold}[% bold upright typewriter font in boldmath.
%    	  version=bold,
%    	  Scale=MatchUppercase,
%          Extension=.otf,    
%    ]
	%
    \setmathfont{LucidaBrightMathOT}[%
    	  range={scr},% to make scr differ from cal
    	  RawFeature={-ss04},
    	  Scale=MatchUppercase,
          Extension=.otf,
    	  BoldFont=LucidaBrightMathOT-Demi.otf,% could be overridden by bold separate version
    ]
    \setmathfont{LucidaBrightMathOT}[% -Demi .. sufficient this way, since bold set above.
    	  range={bfscr},% need to call \symbfscr manually - bug in unicode-math version & range interaction
    	  RawFeature={-ss04},
    	  Scale=MatchUppercase,
          Extension=.otf,
    	  BoldFont=LucidaBrightMathOT-Demi.otf,
    ]
    %% Fix unicode-math operator font not set up for bold face (default \mathrm). See https://github.com/wspr/unicode-math/issues/468
    \setoperatorfont\normalfont
    %
    % note \mathbfit = \symbfit
    
    % The specialized one-off Lucida fonts:
    \newfontface\LucidaBlackletter{LucidaBlackletterOT}[%
    	Scale=0.95,% <== NB
    	Extension=.otf,
    	]
    \newfontface\LucidaCalligraphy{LucidaCalligraphyOT}[%
    	Scale=MatchUppercase,
    	Extension=.otf,
    	]
    \newfontface\LucidaHandwriting{LucidaHandwritingOT}[%
    	Scale=MatchUppercase,
    	Extension=.otf,
     	]
    % GrandeMono and Console fonts:
    \newfontface\LucidaGrandeMonoDK{LucidaGrandeMonoDK}[%	
    	Scale=MatchUppercase,
    	Extension=.otf,
        UprightFont=*,
        ItalicFont=*-Italic,
        BoldFont=*-Bold,
        BoldItalicFont=*-BoldItalic,
    	]
    \newfontface\LucidaConsole{LucidaConsoleDK}[%
    	Scale=MatchLowercase,% <=== NB
    	Extension=.otf,
        UprightFont=*,
        ItalicFont=*-Italic,
        BoldFont=*-Bold,
        BoldItalicFont=*-BoldItalic,
    	]
\fi


==> fontsets/mitthesis-newtx-sans-text.tex <==
% From mitthesis package
% Version: 1.01, 2023/07/03
% Documentation: https://ctan.org/pkg/mitthesis


%% newtx package with sans-serif text (Helvetica-like text with Times-like math)
%
\ifpdftex
	\RequirePackage[T1]{fontenc}
    \RequirePackage[subscriptcorrection,varvw,helvratio=0.91,defaultsups]{newtx}% upint for upright integrals
    \renewcommand{\familydefault}{\sfdefault}% use sans for main text
%   these two commands enable hyphenation of the typewriter font - https://tex.stackexchange.com/a/204421/119566
%    \input{t1ntxtt.fd}
%    \DeclareFontFamily{\encodingdefault}{\ttdefault}{\hyphenchar\font=`\-} % 
	\RequirePackage{bm}% bold math
\else
	\ClassWarning{mitnewthesis}{The newtx font set requires pdflatex.  Defaulting to LMR fonts}
    \RequirePackage[warnings-off={mathtools-colon,mathtools-overbracket}]{unicode-math}
    % suppress tiresome warnings about lack of integration between mathtools and unicode-math.
    % Unicode-math loads the fontspec package, but the default fonts are not selected by fontspec in this case.
\fi

	

==> fontsets/mitthesis-newtx.tex <==
% From mitthesis package
% Version: 1.02, 2023/07/03
% Documentation: https://ctan.org/pkg/mitthesis


\ifpdftex
	\typeout{^^JLoading newtx fonts with inconsolata typewriter^^J}
	\RequirePackage[T1]{fontenc}
    \RequirePackage[subscriptcorrection,varvw,helvratio=0.91]{newtx}% stix2, upint
    \RequirePackage[varl,varqu,hyphenate,mono]{inconsolata}% sans typewriter font; mono = fixed word spacing, hyphenate = allow hyphenation 
	\RequirePackage{bm}
	\let\textsuperscript\textsu% newtx changes the default superiors font; this is needed to get commas aligned in sequential footnotes
\else
	\ClassWarning{mitnewthesis}{The newtx font set requires pdflatex.  Defaulting to LMR fonts}
    \RequirePackage[warnings-off={mathtools-colon,mathtools-overbracket}]{unicode-math}
    % suppress tiresome warnings about lack of integration between mathtools and unicode-math.
    % Unicode-math loads the fontspec package, but the default fonts are not selected by fontspec in this case.
\fi

	

==> fontsets/mitthesis-stix2.tex <==
% From mitthesis package
% Version: 1.02, 2023/07/03
% Documentation: https://ctan.org/pkg/mitthesis


%% STIX Two text and math fonts with Heros sans serif font and Inconsolata monospaced font
%
% These fonts are available at: 
%				https://github.com/stipub/stixfonts 
%				http://www.gust.org.pl/projects/e-foundry/tex-gyre 
%				https://ctan.org/tex-archive/fonts/inconsolata
% Install these as system fonts on your computer
%
\ifpdftex
	\ClassWarning{mitnewthesis}{The stix2 fontset requires a unicode engine. Defaulting to CMR fonts.}
	\RequirePackage[T1]{fontenc}	
	\RequirePackage{bm}
\else
	\typeout{^^JLoading STIX Two text and math fonts with Heros sans serif font and Inconsolata monospaced font.^^J}
	%
    \RequirePackage[warnings-off={mathtools-colon,mathtools-overbracket}]{unicode-math}
    % suppress tiresome warnings about lack of integration between mathtools and unicode-math
    % unicode-math loads the fontspec package
	%
    \setmainfont{STIXTwoText}[% Presumes these are system fonts! 
       	Extension = .otf,
    	UprightFont = *-Regular,
    	ItalicFont = *-Italic,
    	BoldFont = *-Bold,
    	BoldItalicFont = *-BoldItalic,
		SlantedFont = *-Italic,
	]
	\setsansfont{texgyreheros}[% Presumes these are system fonts! 
		WordSpace = {1,1.4,1},
		Extension = .otf,
    	UprightFont = *-regular,
    	ItalicFont = *-italic,
    	BoldFont = *-bold,
    	BoldItalicFont = *-bolditalic,
		Numbers = Lining,
    	Scale=0.91,% 
	]        
	\setmonofont{Inconsolatazi4}[% This otf font ships with the LaTeX Inconsolata package (it's in TeX Live)
        Scale=1.05,%
        Extension = .otf,
        UprightFont = *-Regular,
        ItalicFont = *-Regular,% has no italic face
        BoldFont = *-Bold, 
    	BoldItalicFont = *-Bold,% has no bold italic face
        RawFeature = {+ss01,+ss02,+ss03},
    ]             
	\setmathfont{STIXTwoMath-Regular}[% nice glyphs, but \mkern sometimes needed
    	Scale=MatchUppercase,
    	Extension = .otf,
		BoldFont = *,% STIX Two Math has no bold face
%       Color=NavyBlue, 
    	RawFeature = {+ss01, -ss02, -ss08},
   ]
   % ss01 -- switch calligraphic to script; +ss02 -- variants of g, u, v, w, z; +ss08 -- upright integrals
   %
   \newcommand*{\FRAC}[1]{{\addfontfeature{Fractions=On}#1}}% use OpenType feature for fractions, \FRAC{1/2} 
\fi


==> fontsets/mitthesis-termes-stix2.tex <==
% From mitthesis package
% Version: 1.02, 2023/07/03
% Documentation: https://ctan.org/pkg/mitthesis


%% TeX Gyre Termes text font and Heros sans serif font with STIX2 math font and Inconsolata monospaced font
%
% These fonts are available at: 
%				http://www.gust.org.pl/projects/e-foundry/tex-gyre 
%				https://github.com/stipub/stixfonts 
%				https://ctan.org/tex-archive/fonts/inconsolata
% Install these as system fonts on your computer
%
\ifpdftex
	\ClassWarning{mitnewthesis}{The termes-stix2 fontset requires a unicode engine. Defaulting to CMR fonts.}
	\RequirePackage[T1]{fontenc}	
	\RequirePackage{bm}
\else
	\typeout{^^JLoading TeX Gyre Termes text font with STIX2 math font, Heros sans serif font, and Inconsolata monospaced font.^^J}
	%
    \RequirePackage[warnings-off={mathtools-colon,mathtools-overbracket}]{unicode-math}
    % suppress tiresome warnings about lack of integration between mathtools and unicode-math
    % unicode-math loads the fontspec package
	%
    \setmainfont{TeXGyreTermesX}[% Presumes these are system fonts! Available at: http://www.gust.org.pl/projects/e-foundry/tex-gyre
		WordSpace = {1,1.4,1},%% This stretch matches newtxtext a little better. 1.4
    	Extension = .otf,
    	UprightFont = *-Regular,
    	ItalicFont = *-Italic,
    	BoldFont = *-Bold,
    	BoldItalicFont = *-BoldItalic,
		SlantedFont = *-Italic,
		Numbers = Lining,
	]
	\setsansfont{texgyreheros}[% Presumes these are system fonts! Available at: http://www.gust.org.pl/projects/e-foundry/tex-gyre
		WordSpace = {1,1.4,1},
		Extension = .otf,
    	UprightFont = *-regular,
    	ItalicFont = *-italic,
    	BoldFont = *-bold,
    	BoldItalicFont = *-bolditalic,
		Numbers = Lining,
    	Scale=0.91,% same as for newtx; former value 0.9 too small 2022/01/15
	]        
	\setmonofont{Inconsolatazi4}[% This otf font ships with the LaTeX Inconsolata package (it's in TeX Live)
        Scale=1.05,% rescaled from 1, 22/03/10
        Extension = .otf,
        UprightFont = *-Regular,
        ItalicFont = *-Regular,% has no italic face
        BoldFont = *-Bold, 
    	BoldItalicFont = *-Bold,% has no bold italic face
        RawFeature = {+ss01,+ss02,+ss03},
    ]             
	\setmathfont{STIXTwoMath-Regular}[% nice glyphs, but \mkern sometimes needed %% https://github.com/stipub/stixfonts
    	Scale=MatchUppercase,
    	Extension = .otf,
		BoldFont = *,% STIX Two Math has no bold face
%       Color=NavyBlue, 
    	RawFeature = {+ss01, -ss02, -ss08},
   ]
   % ss01 -- switch calligraphic to script; +ss02 -- variants of g, u, v, w, z; +ss08 -- upright integrals
   %
   \setmathfontface\mathbf{STIXTwoText-Bold.otf}[]% to not get Termes bold, https://github.com/stipub/stixfonts
   \setmathfontface\mathit{STIXTwoText-Italic.otf}[]
   \setmathfontface\mathrm{STIXTwoText-Regular.otf}[]% to get roman letters from STIX, not Termes
    %      
   \newcommand*{\FRAC}[1]{{\addfontfeature{Fractions=On}#1}}% use OpenType feature for fractions, \FRAC{1/2} 
\fi


==> fontsets/mitthesis-termes.tex <==
% From mitthesis package
% Version: 1.02, 2023/07/03
% Documentation: https://ctan.org/pkg/mitthesis


%% TeX Gyre Termes (Times-like) text font with Termes math font and Heros sans serif font and Cursor monospaced font
%
% These fonts are available at: http://www.gust.org.pl/projects/e-foundry/tex-gyre
% install these as system fonts on your computer
%
\ifpdftex
	\ClassWarning{mitnewthesis}{The termes fontset requires a unicode engine. Defaulting to CMR fonts.}
	\RequirePackage[T1]{fontenc}	
	\RequirePackage{bm}
\else
	\typeout{^^JLoading TeX Gyre Termes text and math fonts, Heros sans serif font, and Cursor monospaced font^^J}
    \RequirePackage[warnings-off={mathtools-colon,mathtools-overbracket}]{unicode-math}
    % suppress tiresome warnings about lack of integration between mathtools and unicode-math
    % unicode-math loads the fontspec package
	%
    \setmainfont{TeXGyreTermesX}[% Presumes these are system fonts! Available at: http://www.gust.org.pl/projects/e-foundry/tex-gyre
		WordSpace = {1,1.4,1},
    	Extension = .otf,
    	UprightFont = *-Regular,
    	ItalicFont = *-Italic,
    	BoldFont = *-Bold,
    	BoldItalicFont = *-BoldItalic,
		SlantedFont = *-Italic,
		Numbers = Lining,
	]
    \setsansfont{texgyreheros}[% Presumes these are system fonts! Available at: http://www.gust.org.pl/projects/e-foundry/tex-gyre
		WordSpace = {1,1.4,1},
		Extension = .otf,
    	UprightFont = *-regular,
    	ItalicFont = *-italic,
    	BoldFont = *-bold,
    	BoldItalicFont = *-bolditalic,
		Numbers = Lining,
    	Scale=0.91,% same as for newtx; former value 0.9 too small 2022/01/15
	]        
   \setmonofont{texgyrecursor}[% Presumes these are system fonts! Available at: http://www.gust.org.pl/projects/e-foundry/tex-gyre
        Scale=0.97,
        Extension = .otf,
        UprightFont = *-Regular,
        ItalicFont = *-Italic,
        BoldFont = *-Bold, 
    	BoldItalicFont = *-BoldItalic,
%		BoldFeatures = { Color = VioletRed3 },
    ]             
    \setmathfont{texgyretermes-math}[% Presumes these are system fonts! Available at: http://www.gust.org.pl/projects/e-foundry/tex-gyre
    	Scale=MatchUppercase,
    	Extension = .otf,
		BoldFont = *, % termes-math does not have a bold version
%       Color=Red3, 
    ]
    %   
    \newcommand*{\FRAC}[1]{{\addfontfeature{Fractions=On}#1}}% use OpenType feature for fractions, \FRAC{1/2}
\fi


==> mydesign.tex <==
% From mitthesis package
% Version: 1.00, 2023/06/17
% Documentation: https://ctan.org/pkg/mitthesis


%%%%%%%%%%  Color support  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% Color package: xcolor. 
%% Change this if you prefer something else

%% Options for xcolor
\ifpdftex\def\MyColorOption{fixpdftex}\else\ifluatex\def\MyColorOption{luatex}\else\ifxetex\def\MyColorOption{xetex}\else\def\MyColorOption{}\fi\fi\fi

%\usepackage[hyperref,\MyColorOption,dvipsnames,svgnames,x11names]{xcolor}

\usepackage[hyperref,dvipsnames,svgnames,x11names]{xcolor}
%% can add option [table] to xcolor to use color in tables (see xcolor documentation)


%%%%%%%%%  Caption support  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% 
% see documentation for details of how to customize captions

\RequirePackage{caption}
\RequirePackage{subcaption}


%%%%%%%%%  Customize list environments  %%%%%%%%%%%%%%%%%%%%
% 
% see documentation for details of how to customize lists

%\RequirePackage{enumitem}


%%%%%%%%%  Customize titles and section headings  %%%%%%%%%%
% 
% see documentation for details of how to customize headings

\RequirePackage{titlesec}

% these titlesec commands just automate the bold math in some headings (rest follows default styles)
\titleformat{\section}{\mathversion{bold}\normalfont\Large\bfseries}{\thesection }{1em}{}
\titleformat{\subsection}{\mathversion{bold}\normalfont\large\bfseries}{\thesubsection}{1em}{}
\titleformat{\subsubsection}{\mathversion{bold}\normalfont\normalsize\bfseries}{\thesubsubsection}{1em}{}

% ==> NOT every font includes a bold math version, so you may need to use other math macros in the headings to get bold math <==


%%%%%%%%%  Change page margins  %%%%%%%%%%%%%%%%%%%%%%%%%%%%
% 
% The default thesis margin is 1 inch all around. You may want different margins (e.g., to add a gutter for binding),
% in which case you can use the \newgeometry command from the geometry package.  Refer to the package documentation
% for details.
%
% mitthesis defaults: [top=1in,bottom=1in,left=1in,right=1in,marginparwidth=50pt,headsep=12pt,footskip=0.5in]
%
% The following tells the geometry package to use a two-sided layout with a 1 cm binding offset on the inside 
% 	and 1 inch margins all around, reducing textwidth slightly (by 0.7 cm). See geometry documentation, Section 8.2.
%
%\newgeometry{twoside, bindingoffset=1cm,margin=1in,marginparwidth=50pt,headsep=12pt,footskip=0.5in}

